When Predictions Shape Reality: A Socio-Technical Synthesis of Performative Predictions in Machine Learning

Machine learning models are increasingly used in high-stakes domains where their predictions can actively shape the environments in which they operate, a phenomenon known as performative prediction. This dynamic, in which the deployment of the model influences the very outcome it seeks to predict, can lead to unintended consequences, including feedback loops, performance issues, and significant societal risks. While the literature in the field has grown rapidly in recent years, a socio-technical synthesis that systemises the phenomenon concepts and provides practical guidance has been lacking. This Systematisation of Knowledge (SoK) addresses this gap by providing a comprehensive review of the literature on performative predictions. We provide an overview of the primary mechanisms through which performativity manifests, present a typology of associated risks, and survey the proposed solutions offered in the literature. Our primary contribution is the ``Performative Strength vs. Impact Matrix" assessment framework. This practical tool is designed to help practitioners assess the potential influence and severity of performativity on their deployed predictive models and select the appropriate level of algorithmic or human intervention.

==> Chapters/Key-concepts.tex <==
\section{Key Concepts}

\textbf{Performative Prediction} represents the notion that machine learning models' predictions don't just passively forecast an outcome, but actively influence or cause that outcome. The very action of making a prediction changes the environment in which the model operates, and in turn changes the data that the subsequent iterations of the model will face in the future \citep{perdomo_performative_2020}.

\textbf{Distribution map $D(\theta)$} is a function that uses the parameters of a predictive model $(\theta)$ and maps them to a new data distribution that emerges after the model has been deployed and its predictions influence the environment \citep{peet-pare_long_2022}.

\textbf{Performative Risk} (PR) is a measure of a model's performance that explains the fact that the model's predictions and actions taken based on these predictions can change the data distribution from which future data will be drawn. In a non-performative context, it is assumed that the model relies on a fixed underlying data distribution. In the performative context, this assumption no longer holds as the model itself induces a change in the data distribution. In this case, the Performative Risk of a predictive model with parameters $(\theta)$ is defined as follows:
\[ 
PR(\theta) = \mathbb{E}_{z \sim D(\theta)} \left[ \ell(z; \theta) \right] 
\]
i.e, the performative risk is the expected loss of a predictive model with parameters $(\theta)$, calculated over the data distribution $D(\theta)$ that has been induced by deploying the predictive model.

The notion of Performative Risk has been introduced by \citep{perdomo_performative_2020} to describe the loss function of a predictive model relative to the data distribution created as a result of its deployment. This differs from traditional modelling, which assumes a fixed distribution over its input features and target variable \citep{perdomo_performative_2020}.
Traditionally, the model risk minimisation aims to find a set of model parameters that minimises the loss function over the fixed distribution \citep{perdomo_performative_2023}; however, under conditions of performativity, the aim is to minimise the loss over the distribution created as a result of the model's deployment and not the model's original distribution \citep{peet-pare_long_2022}.




